SuperEncoder: Towards Universal Neural Approximate Quantum State Preparation

Numerous quantum algorithms operate under the assumption that classical data has already been converted into quantum states, a process termed Quantum State Preparation (QSP). However, achieving precise QSP requires a circuit depth that scales exponentially with the number of qubits, making it a substantial obstacle in harnessing quantum advantage. Recent research suggests using a Parameterized Quantum Circuit (PQC) to approximate a target state, offering a more scalable solution with reduced circuit depth compared to precise QSP. Despite this, the need for iterative updates of circuit parameters results in a lengthy runtime, limiting its practical application. In this work, we demonstrate that it is possible to leverage a pre-trained neural network to directly generate the QSP circuit for arbitrary quantum state, thereby eliminating the significant overhead of online iterations. Our study makes a steady step towards a universal neural designer for approximate QSP.

==> 1-background-bak.tex <==
\section{Preliminaries}

In this section, we commence by some basic concepts about quantum computing~\cite{nielsen2010qc-and-qi},
and then proceed to a brief retrospect about existing methods for QSP. 

\subsection{Quantum Computation}

%-------- what is qubit, what is state, what is gate. Describe how $\theta$ impacts qubit state in bloch sphere.

% Quantum mechanics operates in the Hilbert space $\mathcal{H}$

We use Dirac notation throughout this paper. A \emph{pure quantum state} is defined by a vector $|\cdot\rangle$ named `ket', with the unit length.
A state can be written as $|\psi\rangle = \sum_{j=1}^{d} \alpha_j |j\rangle$ with $\sum_{j} |\alpha_j|^2 = 1$, 
where $|j\rangle$ denotes a computational basis state
and $d$ represents the dimension of the complex vector space.
\emph{Density operators} describe more general quantum states.
Given a mixture of $m$ pure states $\{|\psi_i\rangle\}_{i=1}^{m}$ with probabilities $p_i$ and $\sum_{i}^{m} p_i = 1$,
the density operator $\rho$ denotes the \emph{mixed state} as
$\rho = \sum_{i=1}^{m} p_i | \psi_i\rangle \langle \psi_i |$ with $\mathrm{Tr}(\rho) = 1$,
where $\langle \cdot |$ refers to the conjugate transpose of $|\cdot\rangle$.

The fundamental unit of quantum computation is the quantum bit, or \emph{qubit}.
% Quantum information is typically described using the quantum states of these qubits.
A qubit's state can be expressed as $\psi = \alpha |0\rangle + \beta |1\rangle$.  
Given $n$ qubits, the state is generalized to 
$|\psi\rangle = \sum_{j}^{2^n}|j\rangle$,
where $|j\rangle = |j_1 j_2 \cdots j_n\rangle$ 
with $j_k$ the state of $k$th qubit in computational basis, and $j = \sum_{k=1}^{n}2^{n-k} j_k$.
% In quantum computing, these states undergo manipulation through various quantum operations.
A quantum state evolves from one to another state through \emph{quantum operations} including quantum gates and measurements.
Typical single-qubit gates include the Pauli gates
% \todo{Dirac notation}
% The quantum state is manipulated by quantum operations.
% Typical single-qubit operations include Pauli gates, 
$X\equiv \left[\begin{smallmatrix} 0 & 1 \\ 1 & 0 \end{smallmatrix} \right]$, 
$Y\equiv \left[\begin{smallmatrix} 0 & -i \\ i & 0 \end{smallmatrix} \right]$,
$Z\equiv \left[\begin{smallmatrix} 1 & 0 \\ 0 & -1 \end{smallmatrix} \right]$.
These gates have associated rotation operations 
$R_P(\theta)\equiv \mathrm{e}^{-i\theta P/2}$,
where $\theta$ is the rotation angle and $P\in\{X,Y,Z\}$\footnote{In this paper, $R_z,R_y$ are equivalent to $R_Z,R_Y$.}.
Muti-qubit operations create \emph{entanglement} between qubits, allowing one qubit to interfere with others.
In this work, we focus on the controlled-NOT (CNOT) gate, with the mathematical form of 
$\mathrm{CNOT}\equiv |0\rangle\langle0|\otimes\mathbf{I}_2 + |1\rangle\langle1|\otimes\mathrm{X}$.
% To get classical information from quantum state, one needs to perform quantum measurements.
Quantum measurements extract classical information from quantum states, which is described by a collection $\{M_m\}$ with $\sum_m M_m^\dagger M_m = \mathbf{I}$.
Here $m$ refers to the measurement outcomes that may occur in the experiment, with probability of 
$p(m) = \langle\psi|M_m^\dagger M_m|\psi\rangle$.
The post-measurement state of the system becomes
$M_m|\psi\rangle/p(m)$.

A \emph{quantum circuit} is the graphical representation of a series of quantum operations, which can be mathematically represented by a unitary matrix $U$.
In the NISQ era, PQC plays a significant role as it underpins variational quantum algorithms~\cite{farhi2014quantum_qaoa,vqe_nature_comm}.
Typical PQC has the form of $U(\boldsymbol{\theta}) = \prod_i U_i(\theta_i) V_i$, 
where $\boldsymbol{\theta}$ is its parameter vector, $U_i(\theta_i) = \mathrm{e}^{-i\theta_i P_i / 2}$ with $P_i$ denoting a Pauli gate, 
and $V_i$ denotes a fixed gate such as CNOT.
For example, a PQC composed of $R_y$ gates and CNOT gates is depicted in \figref{example_pqc}.
% depicts a sample PQC composed of .
% An example PQC is shown in \figref{example_pqc}.


% \todo{RX RY...}
% \todo{bloch sphere}

\begin{figure}[ht!]
    \centering
    \scalebox{0.8}{
    \begin{quantikz}
        \lstick{$|0\rangle$} & \gate{R_{y}(\theta_0)}\gategroup[wires=4,steps=4,style={inner sep=6pt}]{}  
        \gategroup[wires=4,steps=1,style={dashed, inner sep=2pt, fill=blue!20},background]{}
        % \lstick{$|0\rangle$} & \gate{R_{y}(\theta_0)}\gategroup[wires=4,steps=4]{}  
        & \ctrl{1}
        \gategroup[wires=4,steps=3,style={dashed, inner sep=2pt, fill=red!20},background]{}
        & \qw & \qw        & \gate{R_{y}(\theta_4)} & \ctrl{1} & \qw       & \qw      & \qw \\
        \lstick{$|0\rangle$} & \gate{R_{y}(\theta_1)}                               
        & \targ{} & \ctrl{1} & \qw    & \gate{R_{y}(\theta_5)} & \targ{}  & \ctrl{1}  & \qw      & \qw \\
        \lstick{$|0\rangle$} & \gate{R_{y}(\theta_2)}                               
        & \qw & \targ{} & \ctrl{1}    & \gate{R_{y}(\theta_6)} & \qw      & \targ{}   & \ctrl{1} & \qw \\
        \lstick{$|0\rangle$} & \gate{R_{y}(\theta_3)}                               
        & \qw & \qw & \targ{}         & \gate{R_{y}(\theta_7)} & \qw      & \qw       & \targ{}\slice{Approximated state of $|\boldsymbol{d}\rangle$}  & \qw 
    \end{quantikz} 
    }
    \caption{An example PQC with two blocks, with each block consisting of a rotation layer (filled blue) plus an entangler layer (filled red).}
    \label{fig:example_pqc}
\end{figure}


\subsection{Quantum State Preparation}
\label{ssec:qsp}

% - mottonen algorithm

% \todo{an example circuit for mottonen}

% - variational QSP.


% - Formalize QSP.
Successful execution of many quantum algorithms requires the initial step of loading classical data into a quantum state~\cite{biamonte2017qml_nature_review,Harrow2009-ai_hhl}, 
a process known as \emph{quantum state preparation}.
This procedure involves implementing a quantum circuit to evolve a system to a designated state. 
Here, we focus on \emph{amplitude encoding} and formalize its procedure as follows.
% a $n$-qubit state from $|0\rangle^{\otimes n}$ to an arbitrary state $|\psi\rangle$.
% In this paper, we focus on the application scenarios of QSP in quantum-enhanced linear algebra~\cite{Harrow2009-ai_hhl} and QML~\cite{biamonte2017qml_nature_review}\todo{citations refresh}.
% These applications require to load classical data into quantum state.
% Then the problem of QSP in this context can be described as: 
% The most straightforward way of precise QSP is \emph{amplitude encoding} (AE).
% Let $\boldsymbol{d}$ be an $N$-dimensional classical vector,
Let $\boldsymbol{d}$ be a real-valued $N$-dimensional classical vector, 
AE encodes $\boldsymbol{d}$ into the amplitudes of an $n$-qubit quantum state $|\boldsymbol{d}\rangle$,
where $N=2^n$.
More specifically, the data quantum state is represented by

\begin{equation}
    |\boldsymbol{d}\rangle = \sum_{j=0}^{N-1} d_j |j\rangle,
\end{equation}

where $d_j$ denotes the $j$th element of the vector $\boldsymbol{d}$, and $|j\rangle$ refers to a computational basis state.
% Given an $n$-qubit ($N=2^n$) system with initial state $|0\rangle^{\otimes n}$, 
The main objective is to generate a quantum circuit $U$
which initializes an $n$-qubit system,


\begin{equation}
    U |0\rangle^{\otimes n} = \sum_{j=0}^{N-1} \alpha_j|j\rangle,
\end{equation}

whose amplitudes $\alpha_j$ are set to be equal to $d_j$.
In general, such a circuit must include a number of gates that scales exponentially with $n$~\cite{mottonen2004pennylane_AME,plesch2011qsp_PRA},
rendering AE impractical, especially in current NISQ era.

Fortunately, many quantum algorithms are compatible with \emph{approximate} QSP~\cite{zoufal2019quantum_gan_npjq}.
Taking this opportunity, \emph{approximate amplitude encoding} has emerged as a promising technique~\cite{zoufal2019quantum_gan_npjq,nakaji2022aae_pr_research,wang2023robuststate}.
Specifically, AAE trains a PQC $U(\boldsymbol{\theta})$ (a.k.a. ansatz) to approximate the target quantum state,
where $\boldsymbol{\theta}$ denotes a vector of free parameters for adaptive optimizations,
following a similar procedure of other variational quantum algorithms~\cite{vqe_nature_comm,farhi2014quantum_qaoa}.
Typical ansatz consists of several blocks of operations with the same structure.
For example, a two-block ansatz with 4 qubits is shown in \figref{example_pqc},
where the rotation layer is composed of single-qubit rotational gates $R_y(\theta_r) = \mathrm{e}^{-i\theta_r Y/2}$,
and the entangler layer comprises CNOT gates.
Note that the entangler layer is configurable and hardware-native, 
which means that we can apply CNOT gates to physically adjacent qubits,
% Note that the connections of CNOT gates can be configured to be \emph{native} to target hardware, 
thereby eliminating the necessity of additional SWAP gates to overcome the topological constraints~\cite{li2019tackling}.
This type of PQC is also known as \emph{hardware-efficient ansatz}~\cite{nature_hw_efficient_ansatz}, 
being widely adopted in previous studies of AAE~\cite{zoufal2019quantum_gan_npjq,nakaji2022aae_pr_research,wang2023robuststate}.


\todo{discuss whether we need this section}
\red{\subsection{Operator Learning}}

\red{Let $D\subset \mathbb{R}^d$ be a bounded, open set and $\mathscr{A}$ and $\mathscr{C}$be separable Banach spaces of functions. An operator is a map $\mathcal{N}:\mathscr{A}\rightarrow\mathscr{C}$, for $f\in\mathscr{A}$ and $g\in\mathscr{C}$, we have $\mathcal{N}(f)=g$. According to universal approximation theorem of operator~\cite{lu2021learning_deeponet_op_learning,operatorapproximation_op_learn}, neural operators were introduced to learning such mappings.  To learn the neural operators we could define a loss function:$\mathcal{L}:\mathscr{C}\times\mathscr{C}\rightarrow \mathbb{R}$, the selection of an appropriate loss function is a crucial step in the learning process of these networks and has a substantial impact on their performance.}


% evolves the state through .
% a quantum circuit $U$ evolves the state through $U |0\rangle^{\otimes n} = \sum_{j=0}^{N-1} \alpha_j|j\rangle$.
% The goal is to find an implementation of $U$ that sets the am
% AE aims at finding an implementation of $U$ to make $\alpha_i = d_i, \forall i \in [0,N-1]$.

%------\todo{below needs refresh}
%------
%------Given an $n$-qubit system, 
%------
%------Let $|\boldsymbol{d}\rangle$ be the target state $n$-qubit state whose amplitude represents the classical data component.
%------Our goal is to implement a quantum circuit $U$, such that $U|0\rangle \to |\boldsymbol{d}\rangle$.
%------This problem is also know as amplitude encoding.
%------ 
%------
%------
%------% - Traditional QSP methods.
%------However, to realize precise amplitude encoding, it is known that we need a quantum circuit with exponential depth with respect to the number of qubits~\cite{mottonen2004pennylane_AME,plesch2011qsp_PRA}\todo{more citation}.
%------
%------% - AAE.
%------
%------To reduce circuit depth, approximate amplitude encoding using PQC has been proposed and explored~\cite{nakaji2022aae_pr_research,zoufal2019quantum_gan_npjq,wang2023robuststate}.
%------In general, these studies follows a similar procedure as follows.
%------Given a classical data represented by real-valued $N$-dimensional vector $\boldsymbol{d}$, first it has to be encoded to the amplitude of an $n$-qubit state $|\boldsymbol{d}\rangle$.
%------More specifically, given $|j\rangle$ as $|j\rangle = |j_1 j_2 \cdots j_n\rangle$ where $j_k$ is the state of the $k$th qubit in computational basis and $j = \sum_{k=1}^n 2^{n-k} j_k$,
%------the data quantum state is given by
%------
%------\begin{equation}
%------    |\boldsymbol{d}\rangle = \sum_{j=0}^{N-1} \boldsymbol{d}_j |j\rangle,
%------\end{equation}
%------
%------where $N=2^n$ and $\boldsymbol{d}_j$ denotes the $j$the element of the vector $\boldsymbol{d}$.
%------Note that here $\boldsymbol{d}$ is normalized, i.e., $\sum_j {\boldsymbol{d}_{j}^2} = 1$.
%------The goal of AAE is to train a PQC $U(\boldsymbol{\theta})$ with $\boldsymbol{\theta}$ the vector of parameters.
%------The state prepared by $U(\boldsymbol{\theta})$ is given by
%------% Given an $N$-dimensional vector $\boldsymbol{a}$, the state prepared by $U(\boldsymbol{\theta})$ is given by 
%------$U(\boldsymbol{\theta}) |0\rangle^{\otimes n} = \sum_{j=0}^{N-1}\boldsymbol{a}_j |j\rangle$, where $\boldsymbol{a}_j$ denotes the $j$th element of a classical data vector $\boldsymbol{a}$ that \emph{approximates} $\boldsymbol{d}$.








==> 2-1-design-method-bak.tex <==
\subsection{Design Methodology}

\label{ssec:design}

% \todo{operator learning}

\begin{figure}
    \begin{subfigure}{0.33\textwidth}
        \includegraphics[width=\linewidth]{figures/mnist_3d_landscape_mse_loss-crop.pdf}
        \caption{$\mathcal{L}_{1}$}
        \label{fig:landscape_mse}
    \end{subfigure}
    \begin{subfigure}{0.33\textwidth}
        \includegraphics[width=\linewidth]{figures/mnist_3d_landscape_state_mse_loss-crop.pdf}
        \caption{$\mathcal{L}_{2}$}
        \label{fig:landscape_state_mse}
    \end{subfigure}
    \begin{subfigure}{0.33\textwidth}
        \includegraphics[width=\linewidth]{figures/mnist_3d_landscape_state_fidelity_loss-crop.pdf}
        \caption{$\mathcal{L}_{3}$}
        \label{fig:landscape_state_fid}
    \end{subfigure}
    
    \caption{Landscape virtualization of different loss functions.}
    \label{fig:landscape}
\end{figure}

\begin{figure}
    \centering
    % \begin{subfigure}{0.4\textwidth}
        \includegraphics[width=0.6\textwidth]{figures/mnist_loss_comparison-crop.pdf}
        \caption{Convergence of different loss functions.}
        \label{fig:loss_comp}
    % \end{subfigure}
\end{figure}


% \begin{figure}
%     \centering
%     \includegraphics[width=0.7\textwidth]{figures/mnist_loss_comparison.pdf}
%     \caption{\todo{tbd}}
%     \label{fig:loss_comp}
% \end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% draft %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \red{We denote the PQC as $f_{QC},$  $$|\psi_{E}\rangle=f_{QC}(|\psi_{T}\rangle),$$ where $|\psi_{T}\rangle$ is the target states and $|\psi_{E}\rangle$ is the encoded states. The function $f_{QC}$ can be parameterized as a vector $\boldsymbol{\theta} = \left\{\theta_1,...\theta_m \right\}$, the size of $\boldsymbol{\theta}$ $m$ is related to the qubits number and structure of PQC. }

% \red{Our goal is to find a universal mapping $f:|\psi_{T}\rangle \rightarrow \boldsymbol{\theta_{T}}.$  }
% % \begin{equation}
%    % \boldsymbol{\theta} = f(|\Psi_{T}\rangle).
% % \end{equation} 
% \red{Due to neural networks can be used to approximate any continuous function, we proposed a SuperEncoder-vanilla to approximate $f$. Specifically, we employ a MLP model to approximate the function $f$ and MSE between the output $\boldsymbol{\hat{\theta}_T}$ and $\boldsymbol{\theta_T}$ as loss function. The $\boldsymbol{\theta_T}$ can be gained by training AAE circuits. }

% \red{We can formulate our task as a recovery of unitary matrix problem. Consider the connection between Schrodinger Equation and unitary matrix, we use operator learning \cite{boulle2023mathematical_guide_op_learn} to solve this problem and propose SuperEnoder-DOP-1 and SuperEncoder-DOP-2. }

% \red{In this paper the operator $\mathcal{N}:\mathscr{H}\rightarrow \mathscr{H},$ where $\mathscr{H}$ represents Hilbert space we want to approximate by neural networks is identity operator $\mathbf{I}$, the input and output function is $f_{QC}.$ Specifically, we sample data $\boldsymbol{x}=\left\{x_1,x_2,...,x_m\right\}$ from some dataset, and use quantum circuit $f_{QC}$ as sensor to evaluate it, the results are denoted as $x_i'$. In this paper, the ideal output of quantum circuit is $f_{QC}(x_i)=x_i$, so the inputs of neural operator $\hat{\mathcal{N}}$ are $\boldsymbol{x}=\left\{x_1,x_2,...,x_m\right\}$. Similarly, the true outputs of the operator on the input function are $\boldsymbol{x}=\left\{x_1,x_2,...,x_m\right\}.$ So the loss function could be defined as $\mathbb{E}[\mathcal{L}(\hat{\mathcal{N}}(\boldsymbol{x})(x_i),x_i)].$ }

% \red{The neural operator $\mathcal{\hat{N}}$ can be decomposed into two parts: the Neural Network (NN) model and the parameterized quantum circuit. The output of the NN model yields the parameters $\boldsymbol{\hat{\theta}}$, and the function $\hat{f}_{QC}$can be constructed by applying these parameters to the quantum circuit. }


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% draft %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% To discuss %
Referring back to the scenario in QML,
we expect that a pre-trained model, 
which we term as \name{}, 
could accurately predict the required parameters based on a given data quantum state (Fig.~\ref{fig:superencoder_workflow}).
However, training such a model is nontrivial.

Let $|\boldsymbol{d}\rangle$ be the target state, and $U(\boldsymbol{\theta})$ be the PQC used in AAE with $\boldsymbol{\theta}$ the trained parameters.
Our goal is to find a universal mapping $f: |\boldsymbol{d}\rangle \rightarrow \boldsymbol{\theta}$.
As neural networks could be used to approximate any continuous function,
the most straightforward solution is to use a neural network to approximate $f$.
Specifically, we employ an MLP model to approximate the function $f$, 
with MSE between the output $\boldsymbol{\hat{\theta}}$ and $\boldsymbol{\theta}$ being the loss function, 
where $\boldsymbol{\theta}$ is gained by training AAE circuits.
We term this method as \name{}-vanilla.

% \todo{compare fidelity superencoder vanilla, DOP, figures show the recovery of vanilla is poor}
However, the effectiveness of \name{}-vanilla is limited.
% \todo{describe performance}
Additionally, this method implies that we need to first generate target parameters using AAE, of which the long runtime hinders pre-training on larger datasets. 
To overcome the drawbacks of \name{}-vanilla, we propose to train a \name{} based on operator learning~\cite{boulle2023mathematical_guide_op_learn}.

% \yilun{discuss below block}


Let $D\subset \mathbb{R}^d$ be a bounded, open set and $\mathscr{A}$ and $\mathscr{C}$be separable Banach spaces of functions. 
An operator is a map $\mathcal{N}:\mathscr{A}\rightarrow\mathscr{C}$, for $f\in\mathscr{A}$ and $g\in\mathscr{C}$, we have $\mathcal{N}(f)=g$. 
According to universal approximation theorem of operator~\cite{lu2021learning_deeponet_op_learning,operatorapproximation_op_learn}, neural operators were introduced to learning such mappings.  
To learn the neural operators we could define a loss function: $\mathcal{L}:\mathscr{C}\times\mathscr{C}\rightarrow \mathbb{R}$, 
the selection of an appropriate loss function is a crucial step in the learning process of these networks and has a substantial impact on their performance~\cite{boulle2023mathematical_guide_op_learn}.

% We can formulate our task as a recovery of unitary matrix problem. 
% Consider the connection between Schrodinger Equation and unitary matrix, we use operator learning \cite{boulle2023mathematical_guide_op_learn} to solve this problem and propose SuperEnoder-DOP-1 and SuperEncoder-DOP-2. 

In this work, we consider the procedure of QSP as a function $f_{U}(|\boldsymbol{d}\rangle)$, 
where $U$ refers to the quantum circuit designated by the target state $|\boldsymbol{d}\rangle$.
Ideally, we have $f_{U}(|\boldsymbol{d}\rangle) = |\boldsymbol{d}\rangle$.
Referring back to the framework of operator learning, 
the input function $f$ and output function $g$ are set to be both $f_{U}$.
That is, $f=g=f_{U}\in \mathscr{H}$.
Therefore, the operator is $\mathcal{N}: \mathscr{H} \rightarrow \mathscr{H}$, essentially an \emph{identity operator} $\mathbf{I}$.

Let $\boldsymbol{\mathcal{D}} = \{|\boldsymbol{d}_1\rangle, |\boldsymbol{d}_2\rangle, \dots, |\boldsymbol{d}_m\rangle\}$
be a dataset consisting of $m$ quantum states.
Our objective is training an operator $\hat{\mathcal{N}}$ that approximates $\mathbf{I}$, for which the training data is given by
% The data for training an operator $\hat{\mathcal{N}}$ to approximate $\mathbf{I}$ is given by 
$\{f_U(|\boldsymbol{d}_1\rangle), f_U(|\boldsymbol{d}_2\rangle), \dots, f_U(|\boldsymbol{d}_m\rangle)\}$.
The output of $\hat{\mathcal{N}}$ is given by 
$\hat{f}_U = \hat{\mathcal{N}}(f_U)$, 
then 
Since the output of $f_U(|\boldsymbol{d}_i\rangle)$ is ideally to be exactly $|\boldsymbol{d}_i\rangle$, 
the dataset that determines $\hat{\mathcal{N}}$ is equivalent to $\boldsymbol{\mathcal{D}}$.

Let $\hat{f}_U = \hat{\mathcal{N}}(f_{U})$ be the output f

% the training data of $\mathcal{N}$ is 
% Following the above framework, we define an operator $\mathcal{N}:\mathscr{H}\rightarrow \mathscr{H}$,
% In this paper the operator $\mathcal{N}:\mathscr{H}\rightarrow \mathscr{H}$,
% where $\mathscr{H}$ denotes Hilbert space.

we want to approximate by neural networks is identity operator $\mathbf{I}$, 
the input and output function is $f_{QC}$. 
Specifically, we sample data $\boldsymbol{x}=\left\{x_1,x_2,...,x_m\right\}$ from some dataset, and use quantum circuit $f_{QC}$ as sensor to evaluate it, 
the results are denoted as $x_i'$. 
In this paper, the ideal output of quantum circuit is $f_{QC}(x_i)=x_i$, 
so the inputs of neural operator $\hat{\mathcal{N}}$ are $\boldsymbol{x}=\left\{x_1,x_2,...,x_m\right\}$. 
Similarly, the true outputs of the operator on the input function are $\boldsymbol{x}=\left\{x_1,x_2,...,x_m\right\}.$ So the loss function could be defined as $\mathbb{E}[\mathcal{L}(\hat{\mathcal{N}}(\boldsymbol{x})(x_i),x_i)].$ 

The neural operator $\mathcal{\hat{N}}$ can be decomposed into two parts: the Neural Network (NN) model and the parameterized quantum circuit. 
The output of the NN model yields the parameters $\boldsymbol{\hat{\theta}}$, and the function $\hat{f}_{QC}$can be constructed by applying these parameters to the quantum circuit. 

\yilun{discuss above block}

With the goal of uncovering the relationship between $|\boldsymbol{d}\rangle$ and $\boldsymbol{\theta}$,
we introduce \name{}, a classical neural network that takes $|\boldsymbol{d}\rangle$ as input and outputs $\boldsymbol{\theta}$.
% The overarching procedure is streamlined, with thre 
Referring back to the scenario in QML, the inference process with \name{} is depicted as Fig.~\ref{fig:superencoder_workflow},
we expect that a pre-trained model could accurately predict the required parameters based on given data quantum state.
However, training such a model is nontrivial.

Particularly, we find it challenging to design a proper loss function for \name{}.
In the remainder of this section, we explore three different designs and analyze their performance.



As an initial exploration, we evaluate the performance of \name{} by applying it to a binary classification task on MNIST dataset and compare the classification accuracy with AAE.
We adopt a simple MLP as the underlying network architecture, the detailed configuration is illustrated in Section~\ref{ssec:setup}.
Let $f(\mathbf{W},|\boldsymbol{d}\rangle)$ be the MLP with $\mathbf{W}$ the model weights. 
The output is given by $\boldsymbol{\hat{\theta}} = f(\mathbf{W},|\boldsymbol{d}\rangle)$.

The first and most straightforward method is \emph{parameter-oriented} training --- setting the loss function $\mathcal{L}_1$ as the MSE between target parameters $\boldsymbol{\theta}$ from AAE and output parameters $\boldsymbol{\hat{\theta}}$ from \name{}.
However, training with $\mathcal{L}_1$ results in notable accuracy degradation as shown in Table~\ref{tab:acc_mnist_initial}.
Additionally, utilizing $\mathcal{L}_1$ implies that we need to first generate labels using AAE, of which the long runtime hinders pre-training on larger dataset. 
Consequently, required is a more effective loss function design without involving AAE.


\yilun{Below table needs fidelity comparison and mnist figure comparison.}
\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|c|c|}
        \hline
        AAE & $\mathcal{L}_1$ & $\mathcal{L}_2$ & $\mathcal{L}_3$ \\
        \hline
        98.01\% & 95.98\% & \todo{tbd} & 97.87\% \\
        \hline
    \end{tabular}
    \caption{\todo{tbd}}
    \label{tab:acc_mnist_initial}
\end{table}

To address this challenge, we propose a \emph{state-oriented} training methodology, that is, using the input of \name{} --- the target quantum state, as the labels.
Since our ultimate goal is to prepare a quantum state $\hat{\psi}$ that approximates the target state $\psi$, we may apply $\boldsymbol{\hat{\theta}}$ to the circuit and execute it to get the prepared state $\hat{\psi}$.
Then it is possible to calculate the difference between $\hat{\psi}$ and $\psi$ as the loss to optimize \name{}.
This approach decouples the training procedure from AAE, being extensible to larger dataset.
We consider two different state-oriented metrics, the first is the MSE between $\hat{\psi}$ and $\psi$, denoted as $\mathcal{L}_2$,
and the second is the \emph{fidelity} of $\hat{\psi}$ relative to $\psi$, expressed as $\mathcal{L}_3 = 1 - |\langle\hat{\psi} |\psi\rangle|^2$.
Results in Table~\ref{tab:acc_mnist_initial} show that $\mathcal{L}_2$ and $\mathcal{L}_3$ achieve competitive accuracy with AAE, verifying that state-oriented training is more effective than parameter-oriented training.

\noindent \textbf{Landscape Analysis}.
To understand the efficacy of these loss functions, we further analyze their landscapes following previous studies~\cite{li2018visualizing_loss_landscape}.
To gain insight from landscape, we plot Fig.~\ref{fig:landscape} using the same scale and color gradients~\cite{christiancmehilwarn2022losslandscapes_blog}.
Compared to state-oriented losses ($\mathcal{L}_2$ and $\mathcal{L}_3$), $\mathcal{L}_1$ has a largely flat landscape with non-decreasing minima, 
thus the model struggles to explore a viable path towards a lower loss value, similar pattern can also be observed in Fig.~\ref{fig:loss_comp}.
In contrast, $\mathcal{L}_2$ and $\mathcal{L}_3$ have much lower minima and successfully converge to smaller loss values.
From Fig.~\ref{fig:landscape}, we can also observe that $\mathcal{L}_3$ has a wider minima than $\mathcal{L}_2$, which may indicate a better generalization capability~\cite{petzka2021relative_flatness_and_generalization_loss}.

\noindent \textbf{Feasibility on Real Devices}.
$\mathcal{L}_2$ relies on $\hat{\psi}$, a pure state that can only be acquired on ideal simulator, preventing its adoption on real quantum devices,
where we only a mixed state $\hat{\rho}$ can be obtained.
In contrast, $\mathcal{L}_3$ can be written as $1 - \langle\psi|\hat{\psi}\rangle\langle\hat{\psi}|\psi\rangle$.
If $\hat{\rho}$ is a pure state, it is equivalent to $|\hat{\psi}\rangle\langle\hat{\psi}|$.
Thus we are able to use a general form of $\mathcal{L}_3$ as follows, on both ideal simulation and noisy real devices. 

\begin{equation}
    \mathcal{L}_3 = 1 - \langle\psi | \hat{\rho} | \psi\rangle.
\end{equation}

\todo{1. first gradient of L. 2. two cases of partial rho partial theta}

On real devices, the mixed state $\hat{\rho}$ can be reconstructed through \emph{quantum tomography}\todo{refs} based on classical shadow. 
Here, for notion simplicity, we denote the quantum tomography process as a transformation $\mathcal{S}$, and denote the measurement expectations of the ansatz as $U(\boldsymbol{\hat{\theta}})$.
Thus the reconstructed density matrix is given by 

\begin{equation}
    \label{eq:hat_rho}
    \hat{\rho} = \mathcal{S}(U(\boldsymbol{\hat{\theta}})).
\end{equation}

%Therefore, we finally choose $\mathcal{L}_3$ as the loss function to optimize \name{}.
Let $\mathbf{W}$ be the weight matrix of MLP, with $k,l$ the element indices.
Then the gradient of the loss function $\mathcal{L}_3$ with respect to $ W_{k,l}$ is 

% \begin{equation}
%     \begin{aligned}
%         % \frac{\partial \mathcal{L}}{\partial  W_{k,l}} &=
%         \nabla_{ W_{k,l}}\mathcal{L}_3 
%         &= 
%         \frac{\partial \mathcal{L}_3}{\partial W_{k,l}} =
%         -\langle \psi|
%         \frac{\partial\hat{\rho}}{\partial W_{k,l}} 
%         |\psi\rangle \\
%         &= 
%         -\langle \psi|
%         \begin{bmatrix}
%             \left(
%             \frac{\partial\hat{\rho}_{1,1}}{\partial\boldsymbol{\hat{\theta}}} 
%             \right)^T
%             % \cdot 
%             \frac{\partial\boldsymbol{\hat{\theta}}}{\partial W_{k,l}}
%             & \cdots & 
%             \left(
%             \frac{\partial\hat{\rho}_{1,N}}{\partial\boldsymbol{\hat{\theta}}} 
%             \right)^T
%             % \cdot 
%             \frac{\partial\boldsymbol{\hat{\theta}}}{\partial W_{k,l}} \\
%             \vdots & \ddots & \vdots \\
%             \left(
%             \frac{\partial\hat{\rho}_{N,1}}{\partial\boldsymbol{\hat{\theta}}} 
%             \right)^T
%             % \cdot 
%             \frac{\partial\boldsymbol{\hat{\theta}}}{\partial W_{k,l}}
%             & \cdots & 
%             \left(
%             \frac{\partial\hat{\rho}_{N,N}}{\partial\boldsymbol{\hat{\theta}}} 
%             \right)^T
%             % \cdot 
%             \frac{\partial\boldsymbol{\hat{\theta}}}{\partial W_{k,l}} \\
%         \end{bmatrix}
%         % \left(
%         % \frac{\partial\hat{\rho}_{i,j}}{\partial\boldsymbol{\hat{\theta}}} 
%         % \cdot 
%         % \frac{\partial\boldsymbol{\hat{\theta}}}{\partial W_{k,l}}
%         % \right)_{i,j}
%         |\psi\rangle,
%     \end{aligned}
% \end{equation}


\begin{equation}
    \begin{aligned}
        % \frac{\partial \mathcal{L}}{\partial  W_{k,l}} &=
        \nabla_{ W_{k,l}}\mathcal{L}_3 
        &= 
        \frac{\partial \mathcal{L}_3}{\partial W_{k,l}} =
        -\langle \psi|
        \frac{\partial\hat{\rho}}{\partial W_{k,l}} 
        |\psi\rangle \\
        &= 
        -\langle \psi|
        \begin{bmatrix}
            \sum_{j=1}^m 
            \frac{\partial\hat{\rho}_{1,1}}{\partial\theta_{j}} 
            % \cdot 
            \frac{\partial\theta_j}{\partial W_{k,l}}
            & \cdots & 
            \sum_{j=1}^m 
            \frac{\partial\hat{\rho}_{1,N}}{\partial\theta_{j}} 
            % \cdot 
            \frac{\partial\theta_j}{\partial W_{k,l}} \\
            \vdots & \ddots & \vdots \\
            \sum_{j=1}^m 
            \frac{\partial\hat{\rho}_{N,1}}{\partial\theta_{j}} 
            % \cdot 
            \frac{\partial\theta_j}{\partial W_{k,l}}
            & \cdots & 
            \sum_{j=1}^m 
            \frac{\partial\hat{\rho}_{N,N}}{\partial\theta_{j}} 
            % \cdot 
            \frac{\partial\theta_j}{\partial W_{k,l}} \\
        \end{bmatrix}
        % \left(
        % \frac{\partial\hat{\rho}_{i,j}}{\partial\boldsymbol{\hat{\theta}}} 
        % \cdot 
        % \frac{\partial\boldsymbol{\hat{\theta}}}{\partial W_{k,l}}
        % \right)_{i,j}
        |\psi\rangle,
    \end{aligned}
\end{equation}
% The gradient of $\boldsymbol{\hat{\theta}}$ with respect to $ W_{k,l}$ is 
While the calculation of $\frac{\partial\boldsymbol{\hat{\theta}}}{\partial W_{k,l}}$ is straightforward, 
obtaining $\frac{\partial\hat{\rho}_{i,j}}{\partial\boldsymbol{\hat{\theta}}}$
is non-trivial.

Suppose an $n$-qubit circuit is parameterized by $m$ parameters $\boldsymbol{\hat{\theta}} = [\hat{\theta}_1, \dots, \hat{\theta}_k, \dots, \hat{\theta}_m]$.
Based on Eq.~\ref{eq:hat_rho}, the gradient of $\hat{\rho}_{i,j}$ with respect to $\hat{\theta}_{k}$ is 
    % $\left(\frac{\partial\mathcal{S}(U(\boldsymbol{\hat{\theta}}))}{\partial U(\boldsymbol{\hat{\theta}})}\right)^T
    % \frac{\partial U(\boldsymbol{\hat{\theta}})}{\partial \theta_j}$.
$\sum_{u}
\frac{\partial\hat{\rho}_{i,j}}{\partial U(\boldsymbol{\hat{\theta}})}
    \frac{\partial U(\boldsymbol{\hat{\theta}})}{\partial \hat{\theta}_k}$.

Here $\frac{\partial\hat{\rho}_{i,j}}{\partial U(\boldsymbol{\hat{\theta}})}$
can be efficiently calculated on classical devices using backpropagation supported by automatic differentiation framework.
However, back-propagation on real quantum devices is infeasible due the No-Cloning theorem~
\cite{nielsen2010qc-and-qi}.
Fortunately, it is possible to utilize the \emph{parameter shift} rule~\cite{crooks2019gradients_param_shift,bergholm2018pennylane_param_shift,wierichs2022general_param_shift} to calculate 
$\frac{\partial U(\boldsymbol{\hat{\theta}})}{\partial \theta_k}$.
In this way, the gradients of the circuit function $U$ with respect to $\theta_j$ are

\begin{equation}
    \begin{aligned}
        \frac{\partial U(\boldsymbol{\hat{\theta}})}{\partial \theta_k}
        &=
        \frac{1}{2}\left(
        U(\theta_{+}) - U(\theta_{-}),
        \right) \\
        \theta_{+} &= [\theta_1,\dots,\theta_k+\frac{\pi}{2},\dots,\theta_m], \\
        \theta_{-} &= [\theta_1,\dots,\theta_k-\frac{\pi}{2},\dots,\theta_m].
    \end{aligned}
\end{equation}

% where $\frac{\partial\hat{\rho}}{\partial\boldsymbol{\hat{\theta}_{i,j}}}$ could be calculated via \emph{parameter shift}\todo{citation}.


==> 6-checklist.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newpage
\section*{NeurIPS Paper Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and precede the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

% %%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This work aims at training-free approximate quantum state preparation. As claimed in the abstract and introduction.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \name{} sacrifices fidelity, as discussed in Section~\ref{ssec:disscuss_future_work}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All these necessary contents for theoretical results are included in Section~\ref{ssec:design}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our code is open-source with instructions to reproduce our results, as described in Section~\ref{ssec:setup}. We also describe the details of experiment settings in Appendix~\ref{sec:impl_detail}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See Section~\ref{ssec:setup}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We illustrate the experimental settings in Section~\ref{ssec:setup}, and provides additional details in Appendix~\ref{sec:impl_detail}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Throughout our experiments, we set the random seed to be fixed for all libraries we used. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We describe the computer resources used in this paper in Section~\ref{ssec:setup}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We have read the code of ethics and followed its requirements.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This work has no societal impact.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper poses no such risks as our released model and datasets are only able to be used for quantum state preparation.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We use an open-source dataset FractalDB, we cite the original paper and indicates the version we use in Section~\ref{ssec:setup}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We submit our assets in zip file and also put them on the anonymous github repository, we have included a README file with detailed descriptions.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}

==> legacy.tex <==
\section{Submission of papers to NeurIPS 2023}


Please read the instructions below carefully and follow them faithfully. \textbf{Important:} This year the checklist will be submitted separately from the main paper in OpenReview, please review it well ahead of the submission deadline: \url{https://neurips.cc/public/guides/PaperChecklist}.


\subsection{Style}


Papers to be submitted to NeurIPS 2023 must be prepared according to the
instructions presented here. Papers may only be up to {\bf nine} pages long,
including figures. Additional pages \emph{containing only acknowledgments and
references} are allowed. Papers that exceed the page limit will not be
reviewed, or in any other way considered for presentation at the conference.


The margins in 2023 are the same as those in previous years.


Authors are required to use the NeurIPS \LaTeX{} style files obtainable at the
NeurIPS website as indicated below. Please make sure you use the current files
and not previous versions. Tweaking the style files may be grounds for
rejection.


\subsection{Retrieval of style files}


The style files for NeurIPS and other conference information are available on
the website at
\begin{center}
  \url{http://www.neurips.cc/}
\end{center}
The file \verb+neurips_2023.pdf+ contains these instructions and illustrates the
various formatting requirements your NeurIPS paper must satisfy.


The only supported style file for NeurIPS 2023 is \verb+neurips_2023.sty+,
rewritten for \LaTeXe{}.  \textbf{Previous style files for \LaTeX{} 2.09,
  Microsoft Word, and RTF are no longer supported!}


The \LaTeX{} style file contains three optional arguments: \verb+final+, which
creates a camera-ready copy, \verb+preprint+, which creates a preprint for
submission to, e.g., arXiv, and \verb+nonatbib+, which will not load the
\verb+natbib+ package for you in case of package clash.


\paragraph{Preprint option}
If you wish to post a preprint of your work online, e.g., on arXiv, using the
NeurIPS style, please use the \verb+preprint+ option. This will create a
nonanonymized version of your work with the text ``Preprint. Work in progress.''
in the footer. This version may be distributed as you see fit, as long as you do not say which conference it was submitted to. Please \textbf{do
  not} use the \verb+final+ option, which should \textbf{only} be used for
papers accepted to NeurIPS. 


At submission time, please omit the \verb+final+ and \verb+preprint+
options. This will anonymize your submission and add line numbers to aid
review. Please do \emph{not} refer to these line numbers in your paper as they
will be removed during generation of camera-ready copies.


The file \verb+neurips_2023.tex+ may be used as a ``shell'' for writing your
paper. All you have to do is replace the author, title, abstract, and text of
the paper with your own.


The formatting instructions contained in these style files are summarized in
Sections \ref{gen_inst}, \ref{headings}, and \ref{others} below.


\section{General formatting instructions}
\label{gen_inst}


The text must be confined within a rectangle 5.5~inches (33~picas) wide and
9~inches (54~picas) long. The left margin is 1.5~inch (9~picas).  Use 10~point
type with a vertical spacing (leading) of 11~points.  Times New Roman is the
preferred typeface throughout, and will be selected for you by default.
Paragraphs are separated by \nicefrac{1}{2}~line space (5.5 points), with no
indentation.


The paper title should be 17~point, initial caps/lower case, bold, centered
between two horizontal rules. The top rule should be 4~points thick and the
bottom rule should be 1~point thick. Allow \nicefrac{1}{4}~inch space above and
below the title to rules. All pages should start at 1~inch (6~picas) from the
top of the page.


For the final version, authors' names are set in boldface, and each name is
centered above the corresponding address. The lead author's name is to be listed
first (left-most), and the co-authors' names (if different address) are set to
follow. If there is only one co-author, list both author and co-author side by
side.


Please pay special attention to the instructions in Section \ref{others}
regarding figures, tables, acknowledgments, and references.


\section{Headings: first level}
\label{headings}


All headings should be lower case (except for first word and proper nouns),
flush left, and bold.


First-level headings should be in 12-point type.


\subsection{Headings: second level}


Second-level headings should be in 10-point type.


\subsubsection{Headings: third level}


Third-level headings should be in 10-point type.


\paragraph{Paragraphs}


There is also a \verb+\paragraph+ command available, which sets the heading in
bold, flush left, and inline with the text, with the heading followed by 1\,em
of space.


\section{Citations, figures, tables, references}
\label{others}


These instructions apply to everyone.


\subsection{Citations within the text}


The \verb+natbib+ package will be loaded for you by default.  Citations may be
author/year or numeric, as long as you maintain internal consistency.  As to the
format of the references themselves, any style is acceptable as long as it is
used consistently.


The documentation for \verb+natbib+ may be found at
\begin{center}
  \url{http://mirrors.ctan.org/macros/latex/contrib/natbib/natnotes.pdf}
\end{center}
Of note is the command \verb+\citet+, which produces citations appropriate for
use in inline text.  For example,
\begin{verbatim}
   \citet{hasselmo} investigated\dots
\end{verbatim}
produces
\begin{quote}
  Hasselmo, et al.\ (1995) investigated\dots
\end{quote}


If you wish to load the \verb+natbib+ package with options, you may add the
following before loading the \verb+neurips_2023+ package:
\begin{verbatim}
   \PassOptionsToPackage{options}{natbib}
\end{verbatim}


If \verb+natbib+ clashes with another package you load, you can add the optional
argument \verb+nonatbib+ when loading the style file:
\begin{verbatim}
   \usepackage[nonatbib]{neurips_2023}
\end{verbatim}


As submission is double blind, refer to your own published work in the third
person. That is, use ``In the previous work of Jones et al.\ [4],'' not ``In our
previous work [4].'' If you cite your other papers that are not widely available
(e.g., a journal paper under review), use anonymous author names in the
citation, e.g., an author of the form ``A.\ Anonymous'' and include a copy of the anonymized paper in the supplementary material.


\subsection{Footnotes}


Footnotes should be used sparingly.  If you do require a footnote, indicate
footnotes with a number\footnote{Sample of the first footnote.} in the
text. Place the footnotes at the bottom of the page on which they appear.
Precede the footnote with a horizontal rule of 2~inches (12~picas).


Note that footnotes are properly typeset \emph{after} punctuation
marks.\footnote{As in this example.}


\subsection{Figures}


\begin{figure}
  \centering
  \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  \caption{Sample figure caption.}
\end{figure}


All artwork must be neat, clean, and legible. Lines should be dark enough for
purposes of reproduction. The figure number and caption always appear after the
figure. Place one line space before the figure caption and one line space after
the figure. The figure caption should be lower case (except for first word and
proper nouns); figures are numbered consecutively.


You may use color figures.  However, it is best for the figure captions and the
paper body to be legible if the paper is printed in either black/white or in
color.


\subsection{Tables}


All tables must be centered, neat, clean and legible.  The table number and
title always appear before the table.  See Table~\ref{sample-table}.


Place one line space before the table title, one line space after the
table title, and one line space after the table. The table title must
be lower case (except for first word and proper nouns); tables are
numbered consecutively.


Note that publication-quality tables \emph{do not contain vertical rules.} We
strongly suggest the use of the \verb+booktabs+ package, which allows for
typesetting high-quality, professional tables:
\begin{center}
  \url{https://www.ctan.org/pkg/booktabs}
\end{center}
This package was used to typeset Table~\ref{sample-table}.


\begin{table}
  \caption{Sample table title}
  \label{sample-table}
  \centering
  \begin{tabular}{lll}
    \toprule
    \multicolumn{2}{c}{Part}                   \\
    \cmidrule(r){1-2}
    Name     & Description     & Size ($\mu$m) \\
    \midrule
    Dendrite & Input terminal  & $\sim$100     \\
    Axon     & Output terminal & $\sim$10      \\
    Soma     & Cell body       & up to $10^6$  \\
    \bottomrule
  \end{tabular}
\end{table}

\subsection{Math}
Note that display math in bare TeX commands will not create correct line numbers for submission. Please use LaTeX (or AMSTeX) commands for unnumbered display math. (You really shouldn't be using \$\$ anyway; see \url{https://tex.stackexchange.com/questions/503/why-is-preferable-to} and \url{https://tex.stackexchange.com/questions/40492/what-are-the-differences-between-align-equation-and-displaymath} for more information.)

\subsection{Final instructions}

Do not change any aspects of the formatting parameters in the style files.  In
particular, do not modify the width or length of the rectangle the text should
fit into, and do not change font sizes (except perhaps in the
\textbf{References} section; see below). Please note that pages should be
numbered.


\section{Preparing PDF files}


Please prepare submission files with paper size ``US Letter,'' and not, for
example, ``A4.''


Fonts were the main cause of problems in the past years. Your PDF file must only
contain Type 1 or Embedded TrueType fonts. Here are a few instructions to
achieve this.


\begin{itemize}


\item You should directly generate PDF files using \verb+pdflatex+.


\item You can check which fonts a PDF files uses.  In Acrobat Reader, select the
  menu Files$>$Document Properties$>$Fonts and select Show All Fonts. You can
  also use the program \verb+pdffonts+ which comes with \verb+xpdf+ and is
  available out-of-the-box on most Linux machines.


\item \verb+xfig+ "patterned" shapes are implemented with bitmap fonts.  Use
  "solid" shapes instead.


\item The \verb+\bbold+ package almost always uses bitmap fonts.  You should use
  the equivalent AMS Fonts:
\begin{verbatim}
   \usepackage{amsfonts}
\end{verbatim}
followed by, e.g., \verb+\mathbb{R}+, \verb+\mathbb{N}+, or \verb+\mathbb{C}+
for $\mathbb{R}$, $\mathbb{N}$ or $\mathbb{C}$.  You can also use the following
workaround for reals, natural and complex:
\begin{verbatim}
   \newcommand{\RR}{I\!\!R} %real numbers
   \newcommand{\Nat}{I\!\!N} %natural numbers
   \newcommand{\CC}{I\!\!\!\!C} %complex numbers
\end{verbatim}
Note that \verb+amsfonts+ is automatically loaded by the \verb+amssymb+ package.


\end{itemize}


If your file contains type 3 fonts or non embedded TrueType fonts, we will ask
you to fix it.


\subsection{Margins in \LaTeX{}}


Most of the margin problems come from figures positioned by hand using
\verb+\special+ or other commands. We suggest using the command
\verb+\includegraphics+ from the \verb+graphicx+ package. Always specify the
figure width as a multiple of the line width as in the example below:
\begin{verbatim}
   \usepackage[pdftex]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.pdf}
\end{verbatim}
See Section 4.4 in the graphics bundle documentation
(\url{http://mirrors.ctan.org/macros/latex/required/graphics/grfguide.pdf})


A number of width problems arise when \LaTeX{} cannot properly hyphenate a
line. Please give LaTeX hyphenation hints using the \verb+\-+ command when
necessary.


\begin{ack}
Use unnumbered first level headings for the acknowledgments. All acknowledgments
go at the end of the paper before the list of references. Moreover, you are required to declare
funding (financial activities supporting the submitted work) and competing interests (related financial activities outside the submitted work).
More information about this disclosure can be found at: \url{https://neurips.cc/Conferences/2023/PaperInformation/FundingDisclosure}.


Do {\bf not} include this section in the anonymized submission, only in the final paper. You can use the \texttt{ack} environment provided in the style file to autmoatically hide this section in the anonymized submission.
\end{ack}



\section{Supplementary Material}

Authors may wish to optionally include extra information (complete proofs, additional experiments and plots) in the appendix. All such materials should be part of the supplemental material (submitted separately) and should NOT be included in the main submission.


\section*{References}

% \citep{wu2019full}


References follow the acknowledgments in the camera-ready paper. Use unnumbered first-level heading for
the references. Any choice of citation style is acceptable as long as you are
consistent. It is permissible to reduce the font size to \verb+small+ (9 point)
when listing the references.
Note that the Reference section does not count towards the page limit.
\medskip
